Towards Building a Robust Toxicity Predictor

Recent NLP literature pays little attention to the robustness of toxicity language predictors, while these systems are most likely to be used in adversarial contexts. This paper presents a novel adversarial attack, \texttt{ToxicTrap}, introducing small word-level perturbations to fool SOTA text classifiers to predict toxic text samples as benign. ToxicTrap exploits greedy based search strategies to enable fast and effective generation of toxic adversarial examples. Two novel goal function designs allow ToxicTrap to identify weaknesses in both multiclass and multilabel toxic language detectors. Our empirical results show that SOTA toxicity text classifiers are indeed vulnerable to the proposed attacks, attaining over 98\% attack success rates in multilabel cases. We also show how a vanilla adversarial training and its improved version can help increase robustness of a toxicity detector even against unseen attacks.

==> 88-06-result-fairness-short.tex <==

\subsection{Results on Unintended Bias Analysis}

To evaluate how  adversarial training methods affect unintended model bias for toxicity text predictors, we analyze the unintended model bias metric and report difference between adversarial trained models versus base models. We draw bar plots showing the Subgroup AUC and BPSN AUC metrics in ~\fref{fig:subgroup_diff_jigsawb} and ~\fref{fig:bpsn_diff_jigsawb} for \Jigsawb, and using ~\fref{fig:subgroup_diff_jigsawm} and ~\fref{fig:bpsn_diff_jigsawm} for \Jigsawm respectively. See data details, metrics and results in \sref{more:bias}. In summary, robust models provide better fairness regarding the two metrics when compared with the base models. 







==> 88-06-result-text-bias.tex <==



\subsection{More Results on Unintended Model Bias}
\label{more:bias}

\paragraph{Experimental Setup for Bias Analysis} The fairness evaluation is done on Jigsaw Unintended Bias dataset published in Toxicity Classification Challenge on Kaggle. It contains 97,320 comments annotated by the Civil Comments Platform. Each comment is labeled with a Toxicity column and a multitude of identity attributes (non-exclusive), which demonstrate the prence of a specific identity in a comment~\citep{DBLP:journals/corr/abs-1909-09758}. Table~\ref{table:gdistribution} shows the distribution of identity labels in the dataset. 

\begin{table}[th]
\centering
\scalebox{0.9}{
\begin{tabular}{|>{\raggedright\arraybackslash}m{1.8cm}cc|}%
\hline%
Identities&Count&Toxic\\
\hline%
male&2053&10.42\\
female&2392&9.03\\
black&699&24.75\\
white&1204&20.76\\
heterosexual&62&9.68\\
homosexual&491&14.87\\
\hline%

\end{tabular}
}
\caption{Distribution of identity groups in Jigsaw. }
\label{table:gdistribution}
\end{table}







\begin{figure*}[ht] 
  \begin{minipage}[b]{0.49\linewidth}
    \centering
    \includegraphics[width=.9\columnwidth]{fig3_binary_subgroup_aucs_diff.pdf}
    \caption{\jigsawb Identity groups Subgroup AUC Differences. Difference of Subgroup AUC scores between adversarial trained \sat, \eat models and the base \jigsawb model.  Score difference is reported for every subgroup (x-axis) 
    (Best viewed in color)}
    \label{fig:subgroup_diff_jigsawb}
  \end{minipage}%
  \hfill 
  \begin{minipage}[b]{0.49\linewidth}
    \centering
    \includegraphics[width=.9\columnwidth]{fig4_binary_bpsn_auc_diff.pdf}
    \caption{\jigsawb Identity groups BPSN AUC Differences. Each bar presents the difference between adversarial trained \sat, \eat models' BPSN AUC and the base \jigsawb model's BPSN AUC. 
    Score difference is reported for every subgroup (x-axis)
    (Best viewed in color)}
    \label{fig:bpsn_diff_jigsawb}
  \end{minipage} 
  \begin{minipage}[b]{0.49\linewidth}
    \centering
    \includegraphics[width=.9\columnwidth]{fig5_multilabel_subgroup_aucs_diff.pdf}
    \caption{\jigsawm Identity groups Subgroup AUC Differences. Difference of Subgroup AUC scores between adversarial trained \sat, \eat models and the base \jigsawm model.  Score difference is reported for every subgroup (x-axis) 
    (Best viewed in color)}
    \label{fig:subgroup_diff_jigsawm}
    \vspace{-5mm}
  \end{minipage}%
  \hfill 
  \begin{minipage}[b]{0.49\linewidth}
    \centering
    \includegraphics[width=.9\columnwidth]{fig6_multilabel_bpsn_auc_diff.pdf}
    \caption{\jigsawm Identity groups BPSN AUC Differences. Each bar presents the difference between adversarial trained \sat, \eat models' BPSN AUC and the base \jigsawm model's BPSN AUC. 
    Score difference is reported for every subgroup (x-axis)
    (Best viewed in color)}
    \label{fig:bpsn_diff_jigsawm}
    \vspace{-5mm}
  \end{minipage} 
\end{figure*}


This experiment evaluates base, \sat and \eat models for \Jigsawb, \Jigsawm regarding unintended bias towards six common identity groups: male, female, black, white, heterosexual and homosexual\_gay\_or\_lesbian.
 We use two metrics for unintended bias: Subgroup AUC and BPSN AUC, and calculate each metric for every identity group. 

\textbf{Subgroup AUC.} Subgroup AUC calculates the ROC-AUC score for each of the identity group. It represents model understanding and performance within the group itself. A low value in this metric means the model does a poor job of distinguishing between toxic and non-toxic comments that mention the identity.

\textbf{Background Positive, Subgroup Negative (BNSP)  AUC.} This calculates the AUC on the non-toxic comments from the identity subgroup and the toxic comments from the background that don't mention the identity. A low value in this metric means that the model confuses non-toxic examples that mention the identity with toxic examples that do not.


In  Figure~\ref{fig:subgroup_diff_jigsawb} and ~\ref{fig:bpsn_diff_jigsawb}, we observe improvements of Subgroup AUCs and BPSN AUC scores by \sat-delete and \eat \jigsawb models in all identity groups over the base \jigsawb model, with an average 1.13\% and 0.75\% improvement for Subgroup AUCs and an average 3.76\% and 3.74\% improvement for BPSN AUC. 

\sat-unk trained model improves the Subgroup AUCs and BPSN AUC scores in all but one identity group -heterosexual, with an average of 0.9\% and 2.15\% improvement for Subgroup AUC and BPSN AUC. These observations indicate that the \sat and \eat both improve the \jigsawb model’s fairness level. 

In Figure~\ref{fig:subgroup_diff_jigsawm} and ~\ref{fig:bpsn_diff_jigsawm}, \eat trained \jigsawm model has higher Subgroup AUC and BPSN AUC (average 0.93\% and 2.96\% improvements) across all identity groups, which makes the model less biased compare with the \jigsawm base model. 

\sat trained \jigsawm models have higher Subgroup AUC except for \sat-unk trained \jigsawm model for heterosexual identity group and \sat-delete trained \jigsawm model for black identity group. On average, \sat-unk and \sat-delete trained \jigsawm has 0.41\% and 0.21\% increase over the base \jigsawm model, respectively.

\sat trained \jigsawm models have lower BPSN AUC over the base \jigsawm model across all identity groups, with an average -5.1\% and -2.9\% decrease by \sat-unk and \sat-delete, respectively. 

These observations prove that \eat improves the \jigsawm model’s fairness level while the \sat does not consistently prove to have positive effect on the \jigsawm's fairness. Among \sat, \sat-unk tend to improve the model fairness while \sat-delete worsen it.  

In summary, \eat improves the model fairness for both \jigsawb and \jigsawm models. \sat improves the model fairness for \jigsawb while it have less effect for \jigsawm model.

